Relightful Harmonization: Lighting-aware Portrait Background Replacement

Portrait harmonization aims to composite a subject into a new background, adjusting its lighting and color to ensure harmony with the background scene. Existing harmonization techniques often only focus on adjusting the global color and brightness of the foreground and ignore crucial illumination cues from the background such as apparent lighting direction, leading to unrealistic compositions. We introduce Relightful Harmonization, a lighting-aware diffusion model designed to seamlessly harmonize sophisticated lighting effect for the foreground portrait using any background image. Our approach unfolds in three stages. First, we introduce a lighting representation module that allows our diffusion model to encode lighting information from target image background. Second, we introduce an alignment network that aligns lighting features learned from image background with lighting features learned from panorama environment maps, which is a complete representation for scene illumination. Last, to further boost the photorealism of the proposed method, we introduce a novel data simulation pipeline that generates synthetic training pairs from a diverse range of natural images, which are used to refine the model. Our method outperforms existing benchmarks in visual fidelity and lighting coherence, showing superior generalization in real-world testing scenarios, highlighting its versatility and practicality.

==> figures/compare_lightstage.tex <==
\begin{figure}[ht]
\begin{overpic}[width=0.45\textwidth]{assets/lightstage_vis_short.pdf}
    \put(0,40){Method 1}
    \put(30,95){Method 2}
    \put(50,95){Method 3}
    \put(70,95){Method 4}
    \put(90,95){Method 5}
    \end{overpic}
    \caption{\todo{move to app.}Comparison on light stage.}
    \label{fig:lightstage}
\end{figure}

==> figures/results_compare.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{assets/benchmark_simple.pdf}
    \caption{In-the-wild testing and comparison with the top-two harmonization. \emph{we can show less compairons  here but put in the sub}}
    \label{fig:compare*}
\end{figure*}

==> figures/results_spatial.tex <==
% \begin{figure*}[t]
%     \centering
% \includegraphics[width=0.9\linewidth]{assets/spatial_rotation.pdf}
%     \caption{\todo{PLACEHOLDER} Spatial consistency}
%     \label{fig:compare}
% \includegraphics[width=0.9\linewidth]{assets/temporal.pdf}\caption{\todo{PLACEHOLDER}Temporal manipulation}
% \end{figure*}

\begin{figure*}
\centering
\begin{subfigure}[][][t]{0.99\textwidth}
    \includegraphics[width=\textwidth]{assets/spatial_1.pdf}
    \caption{Spatial.}
    \label{fig:spatial}
\end{subfigure}
% \hfill
\unskip\ \vrule\
\begin{subfigure}[][][t]{0.99\textwidth}
    \includegraphics[width=\textwidth]{assets/temporal_single.pdf}
    \caption{Temporal }
    \label{fig:temporal}
\end{subfigure}
\caption{Real-world testing results}
\label{fig:real_world}
\end{figure*}

==> figures/results_with_reference.tex <==
\begin{figure*}[t]
    \centering
    % \includegraphics[width=0.98\linewidth]{assets/with_reference.pdf}
    \includegraphics[width=0.9\linewidth]{assets/reference_based_short.pdf}
\vspace{-2mm}
    \caption{Our approach is adaptable for reference-based harmonization tasks, allowing user images to be blended into scenes from real portraits. This involves removing the subject from the reference image (\textit{upper left}) to create a background (\textit{lower left}) for composition. The harmonized results (\textit{right}) achieve lighting effects closely resembling those in the reference.}
    \label{fig:compare}
\end{figure*}

==> figures/shadow_effects.tex <==
% \begin{figure}[t]
%     \centering
% \includegraphics[width=\linewidth]{assets/shadow_effects.pdf}
%     \caption{Shadow effects.}
%     \label{fig:compare}
% \end{figure}

==> figures/shadow_remove.tex <==
% \begin{figure*}[t]
%     \centering
% \includegraphics[width=\linewidth]{assets/shadow_remove.pdf}
%     \caption{Shadow removal.}
%     \label{fig:compare}
% \end{figure*}

==> figures/user_study.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{assets/user_study.pdf}
    \caption{User study. Each row represents the fraction of times that raters preferred our results over the baseline methods.}
    \label{fig:user-study}
\end{figure}

==> tables/table_lightstage.tex <==
\begin{table}[t]
% \setlength\aboverulesep{3pt}
% \setlength\belowrulesep{3pt}
\footnotesize
\setlength{\tabcolsep}{3pt}
\centering
\caption{Light Stage test set}
\label{table:lightstage}
\begin{tabular}{lccc}
\toprule
                 & MSE $\downarrow$                & PSNR $\uparrow$                & SSIM $\uparrow$                              \\
\midrule
TR~\cite{pandey2021total} & 0.044(0.057) & 
15.889(4.318) & 
0.757(0.087)                 \\
PCT~\cite{Guerreiro_2023_CVPR}            &
&
& \\
Harmonizer~\cite{Harmonizer}    & 
0.015(0.011)  & 
19.304(2.980) &
0.822(0.077) \\
PIH~\cite{wang2023semi} &
0.018(0.015 )&
18.865(0.087)& 
0.807(0.087)\\
INR~\cite{} &
0.016(0.014) &
19.147(3.353) &
0.823(0.081) \\
Ours          & 
\textbf{0.012(0.010)}  & 
\textbf{20.376(3.068)} & 
\textbf{0.840(0.076)} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table_stocktest.tex <==
\begin{table}[t]
% \setlength\aboverulesep{3pt}
% \setlength\belowrulesep{3pt}
\footnotesize
\setlength{\tabcolsep}{3pt}
\centering
\caption{Stock simulated test set}
\label{table:stock}
\begin{tabular}{lccc}
\toprule
                 & MSE $\downarrow$                & PSNR $\uparrow$                & SSIM $\uparrow$                              \\
\midrule
PCT~\cite{Guerreiro_2023_CVPR} &
0.014(0.010) &
19.647(3.279) &
0.898(0.038)
\\
Harmonizer~\cite{Harmonizer}    & 
0.001(0.007)  & 
21.419(3.506)  & 
0.905(0.039)  \\
PIH~\cite{wang2023semi} &
\\
INR~\cite{} &
\\
Ours          & 
\\
\bottomrule
\end{tabular}
\end{table}
